A Type System For Call-By-Name Exceptions

We present an extension of System F with call-by-name exceptions. The type system is enriched with two syntactic constructs: a union type for programs whose execution may raise an exception at top level, and a corruption type for programs that may raise an exception in any evaluation context (not necessarily at top level). We present the syntax and reduction rules of the system, as well as its typing and subtyping rules. We then study its properties, such as confluence. Finally, we construct a realizability model using orthogonality techniques, from which we deduce that well-typed programs are weakly normalizing and that the ones who have the type of natural numbers really compute a natural number, without raising exceptions.

==> letter.tex <==
Dear Sylvain Lebresne,

Please find enclosed a version of your paper ``A Type System For
Call-by-name Exceptions'' formatted for the Journal.  

Reduced indentations made it necessary to avoid a number of bad line
breaks in the proofs of Lemma 5.9 on page 17, Lemmas 5.10 and 5.13 on
page 18 and also Lemma 17 on pages 19 and 20.  Further changes are: 

Theorem 3.14:  introduced math displays

page 6, before Definition 3.2: added ``as well'' to the sentence.

page 17, before Lemma 5.9: ``a union'' rather than ``an union'' (since
here ``u'' is pronounced ``yu'')

page 17, proof of Lemma 5.9: replaced ``We show each side of the
equality to be proved separately'' by ``We show each inclusion
separately'' (I _think_ that's what you meant)

page 18, Lemma 5.11: had to break the displayed formula

proof of Lemma 5.17: ... the cases that do not belong... (rather than ``does'')

page 21, proof of Theorem 5.19: added missing full stop.

Please check, if these changes are acceptable to you.

I suspect you are not a native speaker of English, hence it may be
useful to have someone who is proofread the paper.  

Sincerely yours,

-- Jürgen Koslowski
   LMCS Layout Editor

